FedDRL: Deep Reinforcement Learning-based Adaptive Aggregation for Non-IID Data in Federated Learning

The uneven distribution of local data across different edge devices (clients) results in slow model training and accuracy reduction in federated learning. Naive federated learning (FL) strategy and most alternative solutions attempted to achieve more fairness by weighted aggregating deep learning models across clients. This work introduces a novel non-IID type encountered in real-world datasets, namely cluster-skew, in which groups of clients have local data with similar distributions, causing the global model to converge to an over-fitted solution. To deal with non-IID data, particularly the cluster-skewed data, we propose FedDRL, a novel FL model that employs deep reinforcement learning to adaptively determine each client's impact factor (which will be used as the weights in the aggregation process). Extensive experiments on a suite of federated datasets confirm that the proposed FedDRL improves favorably against FedAvg and FedProx methods, e.g., up to 4.05% and 2.17% on average for the CIFAR-100 dataset, respectively.

==> 04_analysis.tex <==
\section{Convergence Analysis (1 page)}\label{sec:analysis}
+ Show the bound 
+ Two first impact item
+ Same as FedAvg?
+ A Case for FedRL better (Featured??)
\newpage

==> 06_related.tex <==
\section{Related Work}\label{sec:related}


==> algorithms/fedavg.tex <==
\begin{algorithm}[t]
    \caption{{\textbf{FedAvg Training Algorithm}}}
    \label{algo:fedavg}
    \small
    \Input{$N$ clients with separated data-set, the number of clients performs training each round $K$.}
    \textbf{Server:} Initiate global model $w^{0}$;\\
    \For{communication round $t$ from $0$ to $T$}{
        Select random $K$ clients;\\
        Server sends $K$ copies of $w^{t}$ to these clients;\\
        \For{each client $k$ in $K$ clients \textbf{in parallel}}{
            $w_{k}^{(t,0)} \gets w^{t}$  \\
            Local training in $E$ epochs with batch $b$:\\
             \hskip2.5em
             $w^{t}_k \gets w^{t} - \eta.\frac{1}{b}\sum_{e=1}^{E}\sum_{i = 1}^{\frac{n_k}{b}}\nabla l_i(w_{k}^{(t,i)})$ \\
            Send ($n_k$, $w^{t}_k$) to server;\\
        }
        Server performs weighted aggregation: \\
        \hskip2.5em
        $n \gets \sum^{K}_{k=1}n_k$;
        $w^{t+1} \gets \sum_{k=1}^{K}{\frac{n_k}{n}w^{t}_k}$    
    }
\end{algorithm}

==> macro.tex <==
\newcommand{\tbhline}{\noalign{\hrule height 1pt}}
\newcommand\inner[2]{\langle #1, #2 \rangle}

\newcolumntype{|}{!{\vrule width 0.5pt}}
\newcolumntype{?}{!{\vrule width 1pt}}
\newcolumntype{^}{!{\vrule width 1.2pt}}


\renewcommand{\O}[1]{$\mathcal{O}(#1)$}


\newcommand{\bhline}[1]{\noalign{\hrule height #1}}    
\renewcommand{\algorithmicrequire}{\textbf{Input:}}
\renewcommand{\algorithmicensure}{\textbf{Output:}}    

%\renewcommand{\theenumi}{\ajMaru{enumi}}


% remove end sentences
\algtext*{EndWhile}
\algtext*{EndIf}

\newcommand{\abs}[1]{\lvert #1 \rvert}
\newcommand{\Break}{\textbf{break}}

\newcommand{\argmax}{\mathop{\rm arg~max}\limits}
\newcommand{\argmin}{\mathop{\rm arg~min}\limits}

\newcommand{\cmark}{\ding{51}}%
\newcommand{\xmark}{\ding{55}}%


\newcommand{\twoKperf}{20}
\newcommand{\fourKperf}{30}
\newcommand{\eightKperf}{2}

\newcommand{\iFDK}{\ding{iFDK}}%


% Nice little colorful numbered boxes
\definecolor{myblue}{RGB}{91,155,213}
\definecolor{mydark}{RGB}{0,0,0}
\newcommand*\circled[1]{\color{white}\tikz[baseline=(char.base)]{
		\node[shape=circle,inner sep=0.5pt,fill=myblue] (char) {#1};}\color{black}\,}
\newcommand*\circledempty[1]{\color{black}\tikz[baseline=(char.base)]{
		\node[shape=circle, draw=myblue, thin, inner sep=0.5pt,fill=white] (char) {#1};}\color{black}\,}
		
		
		
\DeclareRobustCommand{\hlcyan}[1]{{\sethlcolor{cyan}\hl{#1}}}
\DeclareRobustCommand{\hllightgray}[1]{{\sethlcolor{lightgray}\hl{#1}}}
\newcommand{\hilight}[1]{\colorbox{yellow}{#1}}


\SetKwInOut{Input}{Input}
\SetKwInOut{Output}{Output\,}
\SetKwInOut{Data}{Data}
\SetKwProg{Tree}{Tree}{}{EndTree}


\newcommand{\rOne}{\ding{\rotatebox{90}{$256^2\times512\rightarrow256^3$}}}%
\newcommand{\rTwo}{\ding{\rotatebox{90}{$256^2\times512\rightarrow512^3$}}}%
\newcommand{\rThree}{\ding{\rotatebox{90}{$256^2\times512\rightarrow1024^3$}}}%
\newcommand{\rFour}{\ding{\rotatebox{90}{$512^2\times512\rightarrow256^3$}}}%
\newcommand{\rFive}{\ding{\rotatebox{90}{$512^2\times512\rightarrow512^3$}}}%
\newcommand{\rSix}{\ding{\rotatebox{90}{$512^2\times512\rightarrow1024^3$}}}%
\newcommand{\rSeven}{\ding{\rotatebox{90}{$1024^2\times512\rightarrow256^3$}}}%
\newcommand{\rEight}{\ding{\rotatebox{90}{$1024^2\times512\rightarrow512^3$}}}%
\newcommand{\rNine}{\ding{\rotatebox{90}{$1024^2\times512\rightarrow1024^3$}}}%


\newcommand{\pluseq}{\mathrel{+}=}
\newcommand{\asteq}{\mathrel{*}=}


\newcommand{\floor}[1]{\left\lfloor #1 \right\rfloor}
\newcommand{\ceil}[1]{\left\lceil #1 \right\rceil}



\newcommand{\appropto}{\mathrel{\vcenter{
  \offinterlineskip\halign{\hfil$##$\cr
    \propto\cr\noalign{\kern2pt}\sim\cr\noalign{\kern-2pt}}}}}

==> rebutal.tex <==
We thank all reviewers. Should the paper be accepted, all comments would be taken into consideration when preparing the final manuscript. 
We first address main questions and follow by answers to other relatively specific concerns:

##1. Motivation of cluster skew##
**[Reviewers-3]**"Is cluster skew significantly different to label skew? Is it not just the explanation of label skew?"
**Answer:** Nguyen

##2.Clarification of RL##
**[Reviewers-1]**"Please comment on the question whether the agent changes the environment and how that may complicate the effective of RL in this application."
**Answer:** (Le)

##3.The effective of Reinforcement Learning##
**[Reviewers-1]**"it is not clear that RL is specifically targeting only the issue focused by the study. It might as well be effective to address other imbalances"
**Answer:** (Nguyen)

**[Reviewers-3]**"Does this method actually work on a non-ideal dataset (not a typical image recognition dataset)"
**Answer:** (Le)

##4. Reviewer-specific concerns##
**[Reviewers-2]**"The paper does not list the specifications of the systems used"
**Answer:** (Nguyen)

**[Reviewers-1,2,3]**"There are some grammar errors in the manuscript"
**Answer:** We are happy to improve the text based on the suggestions.


==> tables/accuracy_full.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
% \usepackage{multirow}
%\usepackage[normalem]{ulem}
%\useunder{\uline}{\ul}{}

\begin{table*}[t]
	\caption{Comparison of prediction accuracy to baseline approaches with different partitioning methods: \textbf{E}: equal, \textbf{N}: non-equal, \textbf{P}: Pareto, \textbf{CE}: Cluster-E, \textbf{CN}: Cluster-NE. The values show the best prediction accuracy that each FL method reaches during training. The best performance results are highlighted in the bold, underlined font. \emph{impr.(a)} and \emph{impr.(b)} are the relative accuracy improvement of FedDRL compared with the best and the worst baseline FL method (in percentage), respectively.  Significant improvements, i.e., more than $1\%$, are also marked in the bold, underlined font.} 
	\label{table:accuracy}
	\centering
	\scriptsize
	\setlength\tabcolsep{4pt} % default value: 6pt
	\resizebox{\textwidth}{!}{%
    \begin{tabular}{@{}cl|lllll|lllll|lllll@{}}
    \toprule
    \multicolumn{2}{l}{}
    & \multicolumn{5}{c}{\textbf{CIFAR-100}}
    & \multicolumn{5}{c}{\textbf{Fashion-MNIST}}
    & \multicolumn{5}{c}{\textbf{MNIST}}             \\
    \cmidrule(lr){3-7}\cmidrule(lr){8-12}\cmidrule(lr){13-17}
    \multicolumn{2}{l}{Partitioning method}
    & \multicolumn{1}{c}{E} & \multicolumn{1}{c}{N} & \multicolumn{1}{c}{P} & \multicolumn{1}{c}{CE} & \multicolumn{1}{c}{CN}     
    &    \multicolumn{1}{c}{E} & \multicolumn{1}{c}{N} & \multicolumn{1}{c}{P} & \multicolumn{1}{c}{CE} & \multicolumn{1}{c}{CN}
    &    \multicolumn{1}{c}{E} & \multicolumn{1}{c}{N} & \multicolumn{1}{c}{P} & \multicolumn{1}{c}{CE} & \multicolumn{1}{c}{CN} \\
    \midrule
    \multirow{5}{*}{\begin{tabular}[c]{@{}c@{}}10\\  clients\end{tabular}}  
    & SingeSet & 80.83          & 81.56         & 75.63          & 68.6           & 72.67          
    & 91.71 & 91.96 & 90.06 & 88.9 & 88.48 
    & 99.57 & 99.53 & 97.65 & 98.87 & 99.01 \\
    \cmidrule(lr){3-17}
    & FedAvg   & 75.10          & 75.02          & 71.5          & 62.18          & 64.6          
    & \textbf{\underline{86.14}} & \textbf{\underline{91.63}} & \textbf{\underline{86.19}} & \textbf{\underline{83.12}} & 82.97 
    & \textbf{\underline{99.19}} & \textbf{\underline{99.51}} & 89.58 & 98.13 & 97.98 \\
    & FedProx  & 72.84          & 76.65         & \textbf{\underline{72.86}} & 62.25          & 66.8           
    & 85.23 & 91.43 & 86.54 & 82.23 & 82.43 
    & 99.04 & 99.44 & 97.23 & 96.89 & 96.88 \\
    & FedDRL   & \textbf{\underline{77.51}} & \textbf{\underline{76.90}} & 72.4           & \textbf{\underline{64.51}} & \textbf{\underline{67.32}} 
    & 85.99 & 91.45 & 86.92 & 82.59 & \textbf{\underline{84.26}} 
    & 99.18 & 99.47 & \textbf{\underline{97.31}} & \textbf{\underline{98.13}} & \textbf{\underline{98.08}} \\
    \cmidrule(lr){3-17}
    & \emph{impr.(a)} & \textbf{\underline{3.21\%}} & 0.33\% & -0.63\% & \textbf{\underline{3.63\%}} & 0.78\%   
    & -0.17\% & -0.20\% & 0.44\% & -0.64\% & \textbf{\underline{1.55\%}} 
    & -0.01\% & -0.04\% & 0.08\% & 0.00\% & 0.10\% \\
    & \emph{impr.(b)} & \textbf{\underline{6.41\%}} & \textbf{\underline{2.51\%}} & \textbf{\underline{1.26\%}} & \textbf{\underline{3.75\%}} & \textbf{\underline{4.21\%}} 
    & 0.89\% & 0.02\% & 0.85\% & 0.44\% & \textbf{\underline{2.22\%}}
    & 0.14\% & 0.03\% & \textbf{\underline{8.63\%}} & \textbf{\underline{1.28\%}} & \textbf{\underline{1.24\%}} \\
    \midrule
    \multirow{5}{*}{\begin{tabular}[c]{@{}c@{}}100 \\ clients\end{tabular}} 
    & SingeSet & 81.34 & 81.59 & 64.55  & 71.26 & 68.73
    & 91.96 & 92.15 & 88.9 & 88.60 & 88.35 
    & 99.52 & 99.54 & 99.26 & 98.79 & 98.82 \\
    \cmidrule(lr){3-17}
    & FedAvg   & 71.98 &  71.58 & 58.29  & 60.95 & 58.17
    & 88.45 & 90.94 & 85.57 & 84.88 & 83.82 
    & \textbf{\underline{99.15}}  &  99.35 & \textbf{\underline{98.86}} & \textbf{\underline{97.89}} & 98.11 \\
    & FedProx  & 72.52 & 72.89 & \textbf{\underline{58.95}}  & 55.55 & 60.53
    & \textbf{\underline{88.51}} & \textbf{\underline{91.0}} & 86.36  & 84.78 & 83.89 
    & 99.11 & 99.36 & 98.74 & 97.87 & \textbf{\underline{98.12}} \\
    & FedDRL   & \textbf{\underline{73.47}} & \textbf{\underline{73.42}} & 58.41  & \textbf{\underline{61.12}}& \textbf{\underline{61.51}}
    & 88.36 & 90.81 & \textbf{\underline{86.65}} &\textbf{\underline{86.71}} & \textbf{\underline{86.69}} 
    & 99.14 & \textbf{\underline{99.37}} & 98.62 & 97.78 & 97.75 \\
    \cmidrule(lr){3-17}
    & \emph{impr.(a)}    & \textbf{\underline{1.31\%}} & \textbf{\underline{2.13\%}} & -0.92\% & 0.28\% & \textbf{\underline{1.62\%}}
    & -0.17\% & -0.21\% & 0.34\% & \textbf{\underline{2.16\%}} & \textbf{\underline{3.34\%}} 
    & -0.01\% & 0.01\% & -0.24\% & -0.14\% & -0.35\%\\
    & \emph{impr.(b)} & \textbf{\underline{2.07\%}} & \textbf{\underline{2.57\%}} & 0.21\% & \textbf{\underline{10.03\%}} & \textbf{\underline{5.74\%}}
    & -0.10\% & -0.14\% & \textbf{\underline{1.26\%}} & \textbf{\underline{2.28\%}} & \textbf{\underline{3.42\%}} 
    & 0.03\% & 0.02\% & -0.12\% & -0.12\% & -0.34\% \\
    \bottomrule
    \end{tabular}
    }
\end{table*}




==> tables/statistic_dataset2.tex <==
\begin{table}[bt]
	\caption{Statistics of partitioned datasets (02).} 
	\label{table:statistic_dataset_02}
	\centering
	\scriptsize
	\setlength\tabcolsep{3pt} % default value: 6pt
	\resizebox{0.5\textwidth}{!}{%
		\begin{tabular}{lclccccccl}
			\toprule
			\multirow{2}{*}{\textbf{\begin{tabular}[c]{@{}c@{}}Dataset\end{tabular}}} & 
			\multirow{2}{*}{\textbf{\begin{tabular}[c]{@{}c@{}}$\#$clients \end{tabular}}} & 
			\multirow{2}{*}{\textbf{\begin{tabular}[c]{@{}c@{}}Partition \\ Method\end{tabular}}} & 
			\multirow{2}{*}{\textbf{\begin{tabular}[c]{@{}c@{}}$\#$training \\ samples\end{tabular}}} & 
			\multicolumn{2}{c}{\textbf{\begin{tabular}[c]{@{}c@{}}Samples/client\end{tabular}}} &
			\multicolumn{2}{c}{\textbf{\begin{tabular}[c]{@{}c@{}}Classes/client\end{tabular}}}
			\\ \cmidrule(lr){5-6} \cmidrule(lr){7-8}
			& & & & \textbf{mean} & \textbf{std} & \textbf{mean} & \textbf{std} 
			\\ \midrule 
            \multirow{5}{*}{MNIST} & \multirow{5}{*}{10} & Equal & 60000 & 6000 & 0 & 2.8 & 0.74 \\
            & & Non-Equal & 60000 & 6000 & 938 & 0.3 & 0.78 \\
            & & Pareto & 25378 & 2537 & 3286 & 2 & 0 \\
            & & Clustered-E & 19600 & 1960 & 0 & 2 & 0 \\
            & & Clustered-NE & 27440 & 2744 & 1590 & 2 & 0 \\
            
            \midrule
            \multirow{5}{*}{\begin{tabular}[c]{@{}c@{}}Fashion-\\MNIST\end{tabular}} & \multirow{5}{*}{10} & Equal & 60000 & 6000 & 0 & 1.7 & 0.45  \\
            & & Non-Equal & 60000 & 6000 & 979 & 4.1 & 0.7 \\
            & & Pareto & 11898 & 1189 & 1742 & 2 & 0 \\
            & & Clustered-E & 20000 & 2000 & 0 & 2 & 0 \\
            & & Clustered-NE & 19682 & 1968 & 153 & 2 & 0 \\
            
            \midrule
            \multirow{5}{*}{CIFAR-100} & \multirow{5}{*}{10} & Equal & 50000 & 5000 & 0 & 19 & 0.44 \\
            & & Non-Equal & 50000 & 5000 & 552 & 18.8 & 2.31 \\
            & & Pareto & 43550 & 4355 & 3904 & 22.8 & 1.07 \\
            & & Clustered-E & 16000 & 1600 & 0 & 20 & 0 \\
            & & Clustered-NE & 20160 & 2016 & 1029 & 20 & 0 \\

            
            \midrule
            \multirow{5}{*}{CIFAR-100} &\multirow{5}{*}{100} & Equal & 50000 & 500 & 0 & 4.9 & 0.3 \\
            & & Non-Equal & 50000 & 500 & 174 & 3.96 & 1.36 \\
            & & Pareto & 10135 & 101 & 242 & 4.87 & 0.33 \\
            & & Clustered-E & 16000& 160 & 0 & 20 & 0 \\
            & & Clustered-NE & 15920 & 159 & 51 & 20 & 0 \\
            
			\bottomrule
		\end{tabular}
	}
	%\vspace{-0.3cm}
\end{table}

==> tables/statistic_dataset3.tex <==
\begin{table}[bt]
	\caption{Statistics of partitioned datasets (03).} 
	\label{table:statistic_dataset_03}
	\centering
	\scriptsize
	\setlength\tabcolsep{3pt} % default value: 6pt
	\resizebox{0.5\textwidth}{!}{%
		\begin{tabular}{lclccccccl}
			\toprule
			\multirow{2}{*}{\textbf{\begin{tabular}[c]{@{}c@{}}Dataset\end{tabular}}} & 
			\multirow{2}{*}{\textbf{\begin{tabular}[c]{@{}c@{}}$\#$clients \end{tabular}}} & 
			\multirow{2}{*}{\textbf{\begin{tabular}[c]{@{}c@{}}Partition \\ Method\end{tabular}}} & 
			\multirow{2}{*}{\textbf{\begin{tabular}[c]{@{}c@{}}$\#$training \\ samples\end{tabular}}} & 
			\multicolumn{2}{c}{\textbf{\begin{tabular}[c]{@{}c@{}}Samples/client\end{tabular}}} &
			\multicolumn{2}{c}{\textbf{\begin{tabular}[c]{@{}c@{}}Classes/client\end{tabular}}}
			\\ \cmidrule(lr){5-6} \cmidrule(lr){7-8}
			& & & & \textbf{mean} & \textbf{std} & \textbf{mean} & \textbf{std} 
			\\ \midrule 
            \multirow{5}{*}{MNIST} & \multirow{5}{*}{10} & Equal & 60000 & 6000 & 0 & 2.7 & 0.64 \\
            & & Non-Equal & 60000 & 6000 & 938 & 7.1 & 0.94 \\
            & & Pareto & 22470 & 2247 & 20254 & 2 & 0 \\
            & & Clustered-E & 19600 & 1960 & 0 & 2 & 0 \\
            & & Clustered-NE & 27440 & 2744 & 1589 & 2 & 0 \\
            
            \midrule
            \multirow{5}{*}{\begin{tabular}[c]{@{}c@{}}Fashion-\\MNIST\end{tabular}} & \multirow{5}{*}{10} & Equal & 60000 & 6000 & 0 & 2 & 0 \\
            & & Non-Equal & 60000 & 6000 & 1131 & 4.2 & 0.97 \\
            & & Pareto & 16718 & 1671 & 2080 & 1.9 & 0.3 \\
            & & Clustered-E & 20000 & 2000 & 0 & 2 & 0 \\
            & & Clustered-NE & 21438 & 2143 & 287 & 2 & 0 \\
            
            \midrule
            \multirow{5}{*}{CIFAR-100} & \multirow{5}{*}{10} & Equal & 50000 & 5000 & 0 & 19.2 & 0.74 \\
            & & Non-Equal & 50000 & 5000 & 645 & 18.6 & 2.37 \\
            & & Pareto & 39775 & 3977 & 3160 & 23.1 & 1.44 \\
            & & Clustered-E & 16000 & 1600 & 0 & 20 & 0 \\
            & & Clustered-NE & 20160 & 2016 & 1029 & 20 & 0 \\

            
            \midrule
            \multirow{5}{*}{CIFAR-100} &\multirow{5}{*}{100} & Equal & 50000 & 500 & 0 & 4.89 & 0.31 \\
            & & Non-Equal & 50000 & 500 & 146 & 38.9 & 9.35 \\
            & & Pareto & 14270 & 142 & 289 & 4.97 & 0.17 \\
            & & Clustered-E & 16000 & 160 & 0 & 20 & 0 \\
            & & Clustered-NE & 16060 & 160 & 56 & 20 & 0 \\
            
			\bottomrule
		\end{tabular}
	}
	%\vspace{-0.3cm}
\end{table}

==> tables/statistics_dataset.tex <==
\begin{table}[bt]
	\caption{Statistics of partitioned datasets (01).} 
	\label{table:statistic_dataset_01}
	\centering
	\scriptsize
	\setlength\tabcolsep{3pt} % default value: 6pt
	\resizebox{0.5\textwidth}{!}{%
		\begin{tabular}{lclccccccl}
			\toprule
			\multirow{2}{*}{\textbf{\begin{tabular}[c]{@{}c@{}}Dataset\end{tabular}}} & 
			\multirow{2}{*}{\textbf{\begin{tabular}[c]{@{}c@{}}$\#$clients \end{tabular}}} & 
			\multirow{2}{*}{\textbf{\begin{tabular}[c]{@{}c@{}}Partition \\ Method\end{tabular}}} & 
			\multirow{2}{*}{\textbf{\begin{tabular}[c]{@{}c@{}}$\#$training \\ samples\end{tabular}}} & 
			\multicolumn{2}{c}{\textbf{\begin{tabular}[c]{@{}c@{}}Samples/client\end{tabular}}} &
			\multicolumn{2}{c}{\textbf{\begin{tabular}[c]{@{}c@{}}Classes/client\end{tabular}}}
			\\ \cmidrule(lr){5-6} \cmidrule(lr){7-8}
			& & & & \textbf{mean} & \textbf{std} & \textbf{mean} & \textbf{std} 
			\\ \midrule 
            \multirow{5}{*}{MNIST} & \multirow{5}{*}{10} & Equal & 60000 & 6000 & 0 & 2.7 & 0.48 \\
            & & Non-Equal & 60000 & 6000 & 1414 & 6.4 & 1.43 \\
            & & Pareto & 30858 & 3086 & 3814 & 2 & 0 \\
            & & Clustered-E & 19600 & 1960 & 9 & 2 & 0 \\
            & & Clustered-NE & 24696 & 2470 & 1261 & 2 & 0 \\
            
            \midrule
            \multirow{5}{*}{\begin{tabular}[c]{@{}c@{}}Fashion-\\MNIST\end{tabular}} & \multirow{5}{*}{10} & Equal & 60000 & 6000 & 0 & 1.9 & 0.3  \\
            & & Non-Equal & 60000 & 6000 & 1600 & 4.6 & 1.13 \\
            & & Pareto & 29186 & 2918 & 2517 & 3.3 & 0.78 \\
            & & Clustered-E & 20000 & 2000 & 0 & 2 & 0 \\
            & & Clustered-NE & 19860 & 1986 & 208 & 2 & 0 \\
            
            \midrule
            \multirow{5}{*}{CIFAR-100} & \multirow{5}{*}{10} & Equal & 50000 & 5000 & 0 & 18.9 & 0.7 \\
            & & Non-Equal & 50000 & 5000 & 1047 & 18.7 & 3.57 \\
            & & Pareto & 39550 & 3955 & 3387 & 22.4 & 1.1 \\
            & & Clustered-E & 16000 & 1600 & 0 & 20 & 0 \\
            & & Clustered-NE & 20160 & 2016 & 1029 & 20 & 0 \\
            
            \midrule
            \multirow{5}{*}{MNIST} & \multirow{5}{*}{100} & Equal & 60000 & 600 & 0 & 2 & 0.4 \\
            & & Non-Equal & 60000 & 600 & 147 & 4.71 & 1.25 \\
            & & Pareto & 42876 & 428 & 1081 & 1.91 & 0.8 \\
            & & Clustered-E & 19200 & 192 & 0 & 2 & 0 \\
            & & Clustered-NE & 19050 & 190 & 16 & 2 & 0 \\
            
            \midrule
            \multirow{5}{*}{\begin{tabular}[c]{@{}c@{}}Fashion-\\MNIST\end{tabular}} &  \multirow{5}{*}{100} & Equal & 60000 & 600 & 0 & 1.92 & 0.27 \\
            & & Non-Equal & 60000 & 600 & 151 & 4.62 & 1.06 \\
            & & Pareto & 32444 & 324 & 910 & 1.92 & 0.27 \\
            & & Clustered-E & 20000 & 200 & 0 & 2 & 0 \\
            & & Clustered-NE & 19772 & 197 & 21 & 2 & 0 \\
            
            \midrule
            \multirow{5}{*}{CIFAR-100} &\multirow{5}{*}{100} & Equal & 50000 & 500 & 0 & 3.94 & 0.24 \\
            & & Non-Equal & 50000 & 500 & 179 & 3.94 & 1.40 \\
            & & Pareto & 13910 & 139 & 301 & 4.94 & 0.23 \\
            & & Clustered-E & 24000 & 240 & 0 & 20 & 0 \\
            & & Clustered-NE & 23320 & 233 & 26 & 20 & 0 \\
            
			\bottomrule
		\end{tabular}
	}
	%\vspace{-0.3cm}
\end{table}

==> tables/testcase.tex <==
% please add the following required packages to your document preamble:
% \usepackage{multirow}
%\renewcommand{\arraystretch}{1.1}
\begin{table}[t]
\caption{Datasets and models used in experiments.}
\label{table:test_case}
\setlength\tabcolsep{3pt} %default value: 6pt
\resizebox{\linewidth}{!}{
%\begin{tabular}{|l|l|l|l|l|}
\begin{tabular}{lllll}
\toprule
\textbf{Dataset} & \textbf{\begin{tabular}[c]{@{}l@{}}\#Train\\ samples\end{tabular}} & \textbf{\begin{tabular}[c]{@{}l@{}}\#Test\\ samples\end{tabular}} & \textbf{\#Classes} & \textbf{Model} \\ \midrule %\hline
MNIST~\cite{Mnist}            & 60000                                                              & 10000                   & 10                 & CNN~\cite{fedavg_mcmahan2017communication}            \\ \midrule %
Fashion-MNIST~\cite{xiao2017fashion}    & 60000                                                              & 10000                   & 10                 & CNN~\cite{fedavg_mcmahan2017communication}            \\ \midrule %
CIFAR-100~\cite{Krizhevsky09}        & 50000                                                              & 10000                   & 100                & VGG-11~\cite{SimonyanZ14a}         \\ \bottomrule
\end{tabular}    
}
%\vspace{-0.1cm}
\end{table}
\normalsize
%\renewcommand{\arraystretch}{1.0}
